An Adaptive Parallel Arc-Length Method

Parallel computing is omnipresent in today's scientific computer landscape, starting at multicore processors in desktop computers up to massively parallel clusters. While domain decomposition methods have a long tradition in computational mechanics to decompose spatial problems into multiple subproblems that can be solved in parallel, advancing solution schemes for dynamics or quasi-statics are inherently serial processes. For quasi-static simulations, however, there is no accumulating 'time' discretization error, hence an alternative approach is required. In this paper, we present an Adaptive Parallel Arc-Length Method (APALM). By using a domain parametrization of the arc-length instead of time, the multi-level error for the arc-length parametrization is formed by the load parameter and the solution norm. By applying local refinements in the arc-length parameter, the APALM refines solutions where the non-linearity in the load-response space is maximal. The concept is easily extended for bifurcation problems. The performance of the method is demonstrated using isogeometric Kirchhoff-Love shells on problems with snap-through and pitch-fork instabilities. It can be concluded that the adaptivity of the method works as expected and that a relatively coarse approximation of the serial initialization can already be used to produce a good approximation in parallel.

==> Figures/FrustrumData.tex <==
% \begin{table}
\centering
\begin{tabular}{lll}
\toprule
\multicolumn{3}{c}{Boundary conditions}\\
\midrule
$\Gamma_1$ & Symmetry\\
$\Gamma_2$ & Free\\
$\Gamma_3$ & Symmetry\\
$\Gamma_4$ & $u_x=u_y=u_z=0$\\
\midrule
\multicolumn{3}{c}{Geometric parameters}\\
\midrule
$H$ & $1$ & $[\text{m}]$\\
$R_1$ & $1$ & $[\text{m}]$\\
$R_2$ & $2$ & $[\text{m}]$\\
$t$ & $0.1$ & $[\text{m}]$\\
\bottomrule
\end{tabular}
\hfill
\begin{tabular}{lll}
\toprule
\multicolumn{3}{c}{Material parameters}\\
\multicolumn{3}{c}{(Incompressible Mooney-Rivlin)}\\
\midrule
$\mu=c_1+c_2$ & $4.225$ & $[\text{N}/\text{mm}^2]$\\
$c_1/c_2$ & 7 & $[-]$\\
\midrule
\multicolumn{3}{c}{Loads}\\
\midrule
$p$ & $1$ & $[\text{N}/\text{m}]$\\
$\lambda$ & variable & $[\text{N}]$\\
\bottomrule
\end{tabular}

% \end{table}


==> Figures/RoofData.tex <==
% \begin{table}
\centering
\begin{tabular}{lll}
\toprule
\multicolumn{3}{c}{Boundary conditions}\\
\midrule
$\Gamma_1,\Gamma_3$ & $u_x=u_y=u_z=0$\\
$\Gamma_2,\Gamma_4$ & Free\\
\midrule
\multicolumn{3}{c}{Geometric parameters}\\
\midrule
$L$ & $508$ & $[\text{mm}]$\\
$R$ & $2540$ & $[\text{mm}]$\\
$t$ & $6.35$ & $[\text{mm}]$\\
$\theta$ & $10$ & $[\text{rad}]$\\
\midrule
\multicolumn{3}{c}{Material parameters}\\
\multicolumn{3}{c}{(Saint-Venant Kirchhoff laminate)}\\
\midrule
$E_{11}$ & $3300$ & $[\text{N}/\text{mm}^2]$\\
$E_{22},E_{33}$ & $1100$ & $[\text{N}/\text{mm}^2]$\\
$G_{12},E_{13}$ & $660$ & $[\text{N}/\text{mm}^2]$\\
$E_{23}$ & $440$ & $[\text{N}/\text{mm}^2]$\\
$\nu_{12},\nu_{13},\nu_{23}$ & $0.25$ & $[-]$\\
Lay-up & $[0/90/0]$ &$[{}^\circ]$\\
\midrule
\multicolumn{3}{c}{Loads}\\
\midrule
$P$ & $10$ & $[\text{N}]$\\
$\lambda$ & variable & $[\text{-}]$\\
\bottomrule
\end{tabular}
% \end{table}


==> Figures/ShellBeamData.tex <==
% \begin{table}
\centering
\begin{tabular}{lll}
\toprule
\multicolumn{3}{c}{Boundary conditions}\\
\midrule
$\Gamma_1$ & $u_x=u_y=u_z=\theta_x=\theta_y=\theta_z=0$\\
$\Gamma_2$ & $u_y=0$\\
$\Gamma_3$ & $u_x, u_y, u_z$ coupled\\
$\Gamma_4$ & $u_y=0$\\
\midrule
\multicolumn{3}{c}{Geometric parameters}\\
\midrule
$L$ & $1$ & $[\text{m}]$\\
$W$ & $0.01$ & $[\text{m}]$\\
$t$ & $0.01$ & $[\text{m}]$\\
\midrule
\multicolumn{3}{c}{Material parameters}\\
\multicolumn{3}{c}{(Saint-Venant Kirchhoff)}\\
\midrule
$E$ & $75\cdot 10^6$ & $[\text{N}/\text{mm}^2]$\\
$\nu$ & $0$ & $[-]$\\
\midrule
\multicolumn{3}{c}{Loads}\\
\midrule
$p$ & 0.1 & $[\text{N}]$\\
$\lambda$ & variable & $[\text{N}]$\\
\bottomrule
\end{tabular}
% \end{table}


==> Figures/SnappingData.tex <==
% \begin{table}
\centering
\begin{tabular}{lll}
\toprule
\multicolumn{3}{c}{Boundary conditions}\\
\midrule
$\Gamma_1$ & $u_x=u_y=0$\\
$\Gamma_2$ & $u_x=0$, $u_y$ coupled\\
Other & Free\\
\midrule
\multicolumn{3}{c}{Geometric parameters}\\
\midrule
$N_X$ & $3$ & $[-]$\\
$N_Y$ & $3$ & $[-]$\\
$a/l$ & $0.3$ & $[-]$\\
$h_B$, $h_T$ & $5t_g$ & $[\text{mm}]$\\
$l$ & $10.0$ & $[\text{mm}]$\\
$t_b$, $t_w$ & $1.5$ & $[\text{mm}]$\\
$t_s$, $t_g$ & $1.0$ & $[\text{mm}]$\\
\midrule
\multicolumn{3}{c}{Material parameters}\\
\multicolumn{3}{c}{(Compressible Neo-Hookean)}\\
\midrule
$E$ & $78$ & $[\text{N}/\text{mm}^2]$\\
$\nu$ & 0.4 & $[-]$\\
\midrule
\multicolumn{3}{c}{Loads}\\
\midrule
$\lambda P$ & variable & $[\text{N}]$\\
\bottomrule
\end{tabular}
% \end{table}


==> gitignore <==
## Core latex/pdflatex auxiliary files:
*.aux
*.lof
*.log
*.lot
*.fls
*.out
*.toc
*.fmt
*.fot
*.cb
*.cb2
.*.lb

## Intermediate documents:
*.dvi
*.xdv
*-converted-to.*
# these rules might exclude image files for figures etc.
# *.ps
# *.eps
# *.pdf

## Generated if empty string is given at "Please type another file name for output:"
.pdf

## Bibliography auxiliary files (bibtex/biblatex/biber):
*.bbl
*.bcf
*.blg
*-blx.aux
*-blx.bib
*.run.xml

## Build tool auxiliary files:
*.fdb_latexmk
*.synctex
*.synctex(busy)
*.synctex.gz
*.synctex.gz(busy)
*.pdfsync

## Build tool directories for auxiliary files
# latexrun
latex.out/

## Auxiliary and intermediate files from other packages:
# algorithms
*.alg
*.loa

# achemso
acs-*.bib

# amsthm
*.thm

# beamer
*.nav
*.pre
*.snm
*.vrb

# changes
*.soc

# comment
*.cut

# cprotect
*.cpt

# elsarticle (documentclass of Elsevier journals)
*.spl

# endnotes
*.ent

# fixme
*.lox

# feynmf/feynmp
*.mf
*.mp
*.t[1-9]
*.t[1-9][0-9]
*.tfm

#(r)(e)ledmac/(r)(e)ledpar
*.end
*.?end
*.[1-9]
*.[1-9][0-9]
*.[1-9][0-9][0-9]
*.[1-9]R
*.[1-9][0-9]R
*.[1-9][0-9][0-9]R
*.eledsec[1-9]
*.eledsec[1-9]R
*.eledsec[1-9][0-9]
*.eledsec[1-9][0-9]R
*.eledsec[1-9][0-9][0-9]
*.eledsec[1-9][0-9][0-9]R

# glossaries
*.acn
*.acr
*.glg
*.glo
*.gls
*.glsdefs
*.lzo
*.lzs

# uncomment this for glossaries-extra (will ignore makeindex's style files!)
# *.ist

# gnuplottex
*-gnuplottex-*

# gregoriotex
*.gaux
*.gtex

# htlatex
*.4ct
*.4tc
*.idv
*.lg
*.trc
*.xref

# hyperref
*.brf

# knitr
*-concordance.tex
# TODO Comment the next line if you want to keep your tikz graphics files
*.tikz
*-tikzDictionary

# listings
*.lol

# luatexja-ruby
*.ltjruby

# makeidx
*.idx
*.ilg
*.ind

# minitoc
*.maf
*.mlf
*.mlt
*.mtc[0-9]*
*.slf[0-9]*
*.slt[0-9]*
*.stc[0-9]*

# minted
_minted*
*.pyg

# morewrites
*.mw

# nomencl
*.nlg
*.nlo
*.nls

# pax
*.pax

# pdfpcnotes
*.pdfpc

# sagetex
*.sagetex.sage
*.sagetex.py
*.sagetex.scmd

# scrwfile
*.wrt

# sympy
*.sout
*.sympy
sympy-plots-for-*.tex/

# pdfcomment
*.upa
*.upb

# pythontex
*.pytxcode
pythontex-files-*/

# tcolorbox
*.listing

# thmtools
*.loe

# TikZ & PGF
*.dpth
*.md5
*.auxlock

# todonotes
*.tdo

# vhistory
*.hst
*.ver

# easy-todo
*.lod

# xcolor
*.xcp

# xmpincl
*.xmpi

# xindy
*.xdy

# xypic precompiled matrices and outlines
*.xyc
*.xyd

# endfloat
*.ttt
*.fff

# Latexian
TSWLatexianTemp*

## Editors:
# WinEdt
*.bak
*.sav

# Texpad
.texpadtmp

# LyX
*.lyx~

# Kile
*.backup

# gummi
.*.swp

# KBibTeX
*~[0-9]*

# TeXnicCenter
*.tps

# auto folder when using emacs and auctex
./auto/*
*.el

# expex forward references with \gathertags
*-tags.tex

# standalone packages
*.sta

# Makeindex log files
*.lpz

